A Survey of Requirements for COVID-19 Mitigation Strategies. Part II: Elicitation of Requirements

The COVID-19 pandemic has influenced virtually all aspects of our lives. Across the world, countries have applied various mitigation strategies, based on social, political, and technological instruments. We postulate that multi-agent systems can provide a common platform to study (and balance) their essential properties. We also show how to obtain a comprehensive list of the properties by "distilling" them from media snippets. Finally, we present a preliminary take on their formal specification, using ideas from multi-agent logics.

==> ethical-guidelines.tex <==
\begin{framed}\sf\small
\noindent
\textbf{Principles: is this the right app to develop?}

\begin{enumerate}
\item Is it \emph{necessary}?

• Yes, it must be developed to save lives (+).

• No, there are better solutions (–).

\item Is it \emph{proportionate}?

• Yes, the gravity of the situation justifies the potential negative impact (+).

• No, the potential negative impact is disproportionate to the situation (–).

\item Is it \emph{sufficiently effective}, \emph{timely}, \emph{popular} and \emph{accurate}?

• Yes, evidence shows that it will work, is timely, will be adopted by enough people and yields accurate data and insights (+).

• No, it does not work well, is available too late or too early, will not be used widely, and is likely to collect data that have false positives and/or false negatives (–).

\item Is it \emph{temporary}?

• Yes, there is an explicit and reasonable date on which it will cease (+).

• No, it has no defined end date (–).
\end{enumerate}

\noindent
\smallskip
\textbf{Requirements: is this app being developed in the right way?}

\begin{enumerate}[start=5]
\item Is it \emph{voluntary}?

• Yes, it is optional to download and install (+).

• No, it is mandatory and people can be penalized for non-compliance (–).

\item Does it \emph{require consent}?

• Yes, people have complete choice over what data are shared and when, and can change this at any time (+).

• No, default settings are to share everything all the time, and this cannot be altered (–).

\item Are the \emph{data kept private} and \emph{users’ anonymity preserved}?

• Yes, data are anonymous and held only on the user’s phone. Others who have been in contact are notified only that there is a risk of contagion, not from whom or where. Methods such as differential privacy are used to ensure this. Cyber-resilience is high (+).

• No, data are (re)identifiable owing to the level of data collected, and stored centrally. Locations of contacts are also available. Cyber-resilience is low (–).

\item Can users \emph{erase the data}?

• Yes, they can do so at will; all data are deleted at the end point (+).

• No, there is no provision for data deletion, nor a guarantee that it can ever be deleted (–).

\item Is the \emph{purpose of data collection} defined?

• Yes, explicitly; for example, to alert users that they have encountered a potentially infected person (+).

• No, the purposes of data collection are not explicitly defined (–).

\item Is the purpose \emph{limited}?

• Yes, it is used for tracing and tracking of COVID-19 only (+).

• No, it can be regularly updated to add extra features that extend its functionality (–).

\item Is it \emph{used only for prevention}?

• Yes, it is used only to enable people voluntarily to limit spread (+).

• No, it is also used as a passport to enable people to claim benefits or return to work (–).

\item Is it used for \emph{compliance}?

• No, it is not used to enforce behaviour (+).

• Yes, non-compliance can result in punishment such as a fine or jail time (–).

\item Is it \emph{open-source}?

• Yes, the code is publicly available for inspection, sharing and collaborative improvement (+).

• No, the source code is proprietary, and no information about it is provided (–).

\item Is it \emph{equally available}?

• Yes, it is free and distributed to anyone (+).

• No, it is arbitrarily given only to some (–).

\item Is it \emph{equally accessible}?

• Yes, it is user-friendly, even for naive users, and works on the widest possible range of mobile phones (+).

• No, it can be used only by those with specific devices and with sufficient digital education (–).

\item Is there a \emph{decommissioning process}?

• Yes, there is a process for shutting it down (+).

• No, there are no policies in place (–).
\end{enumerate}
\end{framed}

